The superconformal index of theories of class $\cal S$

This is the 8th article in the collection of reviews "Exact results in N=2 supersymmetric gauge theories", ed. J. Teschner. The article reviews the superconformal index. It is often simpler to calculate than instanton partition functions, but nevertheless allows one to perform many nontrivial checks of conjectured dualities. It turns out to admit a representation in terms of a new type of topological field theory associated to the Riemann surfaces $C$ parameterising the class $\cal S$ theories.

==> sections/S8.tex <==
\section{Back to the $(2, 0)$ theory}\label{M5sec}

The  expression for the index of theories of class ${\cal S}$ has a very 
uniform structure~\eqref{finindex}. An interesting question is whether the structure
of this expression as a sum over irreps and factors associated to the punctures
has a natural physical meaning.\footnote{This section is based on un-published 
work of the authors with D.~Gaiotto~\cite{GRR6d}.} In this section we will outline
a possible way to interprete such a structure.

The superconformal index counts local operators in $4d$. Since theories of class ${\cal S}$ 
are obtained by dimensionally reducing the $6d$ $(2,0)$ theory one should be able to trace these
operators  to objects in $6d$.  Some of the local operators in $4d$ descend from local operators in $6d$,
but other can come from extended objects in $6d$, surface defects, 
wrapping the Riemann surface ${\cal C}$. Let us 
rewrite thus~\eqref{finindex} in a more uniform form,
\be\label{ind6}
{\cal I}=\sum_{\alpha} (C_\alpha)^{2{\frak g}-2+s}\;
\prod_{i=1}^s \psi_\alpha^{(\Lambda)}(z_i)\,.
\ee The interpretation we propose is that the representation $\alpha$ labels the choice 
of $6d$ surface defect wrapping the Riemann surface with the factors $C_\alpha$ counting the 
states in $4d$ obtained from states on the defect. The functions $\psi_\alpha^{(\Lambda)}(z_i)$
associated to the punctures on the Riemann surface count then states in $6d$ localized at these
singularities. In particular the factor $C_0$ coming from the trivial representation should
correspond to  the local  $6d$ operators. This interpretation is  analogous to what happens
when one reduces from four dimensional theory to a three dimensional one where both theories are known explicitly. For example, when reducing a gauge theory on a circle one can consider line defects
wrapping such a circle. In three dimensions these extended objects, line defects, become {\it local} monopole operators. In particular the index in three dimensions can be written as a sum over GNO charges of such monopole operators with the zero charge sector coming directly from local operators 
in four dimensions and higher charge sectors coming from line defects 
wrapping the $\S^1$.\footnote{
This can be explicitely seen by considering an index of a  $4d$ theory quantized on a manifold with 
a spatial cycle. An example of such a manifold is the lens space $\S^3/{\mathbb Z}_r\times \S^1$ for
which such reductions have been discussed~\cite{Benini:2011nc,Razamat:2013jxa,Razamat:2014pta}.
See also~\cite{Aharony:2013dha,Aharony:2013kma} for a general discussion of $4d/3d$ reductions
and the role of the line defects/monopole operators.
}

\

This suggestion can be made quantitative in the case when the index counts 
operators in a free theory. An example of such a scenario is the limit of large $N$ in which
the protected states counted by the index have a holographic interpretation as free supergravity
modes. In the large $N$ limit the only non-vanishing contribution in~\eqref{ind6} comes from the 
singlet representation~\cite{Gadde:2011uv}. In the large $N$ limit the index of a theory corresponding to genus ${\frak g}$ Riemann surface with no punctures is given by $\left(C_0\right)^{2\frak g-2}$.
We should account for these operators following local operators in $6d$ since the extended objects
become very massive. The reduction from $6d$ to $4d$ is obtained by a topological twist involving
 the angular momentum on the Riemann surface.  Thus, any state in $6d$ which has spin $k$ along
the dimensions of the Riemann surface becomes a degree $k$ differential. By the Riemann-Roch 
theorem there are $(2k-1)(\frak g-1)$ differentials of degree $k$ on a surface of genus $\frak g$.
Thus a spin $k$ operator in $6d$ will reduce to $(2k-1)(\frak g-1)$ operators in $4d$ with other 
quantum numbers shared by the operators in the two theories. We defining the superconformal 
index of the $6d$ theory to be~\cite{Bhattacharya:2008zy} 
\be\label{6dindex}
{\cal I}_{6d}(p,q,t,s)=Tr(-1)^F\,p^{h_1-r}\,q^{h_2-r}\,s^{-h_3-r}\,t^{R+r}\,,
\ee
where $h_i$ re the rotation generators on th three orthogonal planes of $\S^5\times\mathbb R$,
and $(R,r)$ are the R-symmetry charges reducing to the $SU(2)_R\times U(1)_r$ in $4d$. 
One can immediately write the following relation
\be\label{6dpred}
\left(C_0\right)^{2\frak g-2}=
PE\left[
\left.(\frak g-1)\,
(2s\partial_s-1)\,\left\{
(1-s)\,
(I_{6d}^{s.p.}(N\to\infty)-I_{6d}^{s.p.}(N=1)\right\}
\right|_{s=1}
\right]\,.
\ee Here $s$ couples to the angular momentum on the Riemann surface. 
The factor of $(1-s)$ removes the contributions of the derivatives along the surface.
The index of the $(2,0)$ theory in the large $N$ limit was computed in~\cite{Bhattacharya:2008zy},
\bea
&&I_{6d}^{s.p.}(p,q,t,s;N\to\infty)=\frac{(\frac{pqs}{t}+t)(1-pqs)-pqs(\frac1p+\frac1q+\frac1s-p-q-s)}{(1-p)(1-q)(1-s)(1-t)(1-\frac{pqs}{t})}\,,\\
&&I_{6d}^{s.p.}(p,q,t,s;N=1)=\frac{\frac{pqs}{t}+t+pqs-ps-qs-pq}{(1-p)(1-q)(1-s)}\,,\nonumber
\eea
and the coefficient $C_0$ is known explicitly in the Macdonald limit $p=0$~\cite{Gadde:2011uv},
\be
C_0=PE[-\frac{1}{2}\frac{t^2+t\,q}{(1-t)(1-q)}]\,.
\ee  The expression~\eqref{6dpred} thus can be easily checked to hold in the Macdonald limit.
It also can be used as a prediction for $C_0$ for the index depending on all three fugacities $p$, $q$, and $t$.

\

For finite $N$ the $6d$ theory is interacting and the above logic does not strictly hold.
However, in certain cases the index counts operators which do not have any constraints
and thus are not sensitive to the non-trivial dynamics. An example of such an index 
is the Coulomb limit of the $4d$ index~(see section~\ref{secLimits}).  A natural question is whether 
 an analogous limit of the $6d$ index exists. 
An interesting limit of the $6d$
index~\eqref{6dindex} is the analogue of the $4d$ Schur limit, $q=t$.  It can be shown that in this limit
the $6d$ index depends only on $q$ and on the ratio $p/s$.  In the particular cases of single $M5$ brane
or large number of $M5$ branes the index actually depends only on $q$. 
Assuming that in this limit the index counts $6d$ operators generated freely
the equation~\eqref{6dpred} holds for finite $N$. Moreover this equation becomes 
an ordinary  differential equation in the Schur limit ($x=p/s$)
\be
PL[C_0]=(x\partial_x-1)\,(I_{6d}^{s.p.}(q,x;N)-I_{6d}^{s.p.}(q,x;1))\,.
\ee 
We know the left hand side for any value of $N$ in the Schur limit~\cite{Gadde:2011uv} 
and it is independent of $x$. Thus this equation can be easily integrated to give
\be\label{schur6}
I^{s.p.}_{6d}(q;N)=\frac{q + q^2 + \dots q^N}{1-q}\,.
\ee
Interestingly this results agrees with the recent computation of~\cite{Kim:2012ava}.
Moreover,~\eqref{schur6} coincides with truncating the supergravity modes at level $N$, which
is consistent with our assumption that the Schur limit counts effectively free operators.   
Following our general logic the subleading terms $C_\alpha\sim dim_q(\alpha)^{-1}$
count  $4d$ operators descending from surface defects wrapping the Riemann surface in $6d$.
 


\
